ForzaETH Race Stack -- Scaled Autonomous Head-to-Head Racing on Fully Commercial off-the-Shelf Hardware

Autonomous racing in robotics combines high-speed dynamics with the necessity for reliability and real-time decision-making. While such racing pushes software and hardware to their limits, many existing full-system solutions necessitate complex, custom hardware and software, and usually focus on Time-Trials rather than full unrestricted Head-to-Head racing, due to financial and safety constraints. This limits their reproducibility, making advancements and replication feasible mostly for well-resourced laboratories with comprehensive expertise in mechanical, electrical, and robotics fields. Researchers interested in the autonomy domain but with only partial experience in one of these fields, need to spend significant time with familiarization and integration. The ForzaETH Race Stack addresses this gap by providing an autonomous racing software platform designed for F1TENTH, a 1:10 scaled Head-to-Head autonomous racing competition, which simplifies replication by using commercial off-the-shelf hardware. This approach enhances the competitive aspect of autonomous racing and provides an accessible platform for research and development in the field. The ForzaETH Race Stack is designed with modularity and operational ease of use in mind, allowing customization and adaptability to various environmental conditions, such as track friction and layout. Capable of handling both Time-Trials and Head-to-Head racing, the stack has demonstrated its effectiveness, robustness, and adaptability in the field by winning the official F1TENTH international competition multiple times.

==> README <==
# Plotting guidelines

- in case you are using draw.io, save the plot in the drive, link it around and try to follow the same guidelines. You can regulate the proper width based on the page visual dotted guides that appear if you tick View>Page View
- upload all the code and data needed to replicate your plots on the drive, so that everybody can replicate them and apply small changes

- always add units and legends in the plots and make them ultra pretty pls
- plot in pdf, high quality
- Fix the image width, 7 inches for the entire width, 3.5 inches for half width 
- with fixed width, set the fontsize to 8 points, if needed, 6 points for smaller text
- fix the font to Times New Roman
- keep a coherent color scheme throughout the paper. Save any shared color here too:

- JFR guidelines are here: https://media.wiley.com/assets/7323/92/electronic_artwork_guidelines.pdf
[Paper] JFR Full System - F110 Shared Drive - Google Drive

## Jonas consistency guidelines
### Wording
 - self-driving (not self driving or selfdriving)
 - head-to-head (not head to head)
 - racecar (not race car, or robot --> i.e. for consistency try to call the system a race car not a robot)
 - car state (not carstate)
 - racetrack (not race track)
 - racing line (not race line)
### Emphasizing
Emphasize (\emph{}) the following:
 - F1TENTH
 - See-Think-Act
 - ForzaETH
 - Race Stack
 - Frenet
 - Grand-Prix
 - any noun that describes a particular concept or subsystem you want to highlight
Do not emphasize acronyms (you can however emphasize the term for which you are using the acronym: e.g. "Indy Autonomous Challenge (IAC)")
### General Remarks
 -  Use the gls package for abbreviations
 - Use the SI package for units
 - Format multi-line mathematical expressions as equation \begin{equation} ...
 - Use Grammarly (works within overleaf). I corrected a few spelling mistakes that Grammarly would have found.
 - Float Specifiers for Figures, Tables, etc.
 - Use float specifiers [ht]  for figures, tables, etc.
   - h tells latex to place the figure approximately here
   - t tells latex to place the figure at the top of the page
   - ht allows both, whereas latex always first tries to place the figure 'here'
   - H tells latex to place the figure exactly here (might be useful in rare cases)
   - ! tells latex to ignore certain restrictions (like maximum float size, maximum number of floats per page, etc.)
I would therefore generally recommend using [ht], we can still change this for the final layout of the paper wherever needed.


==> chapters/biography.tex <==
\section{Biography Section}
If you have an EPS/PDF photo (graphicx package needed), extra braces are
 needed around the contents of the optional argument to biography to prevent
 the LaTeX parser from getting confused when it sees the complicated
 $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
 your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
 simpler here.)

\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}

==> chapters/ekf_tf.tex <==
\begin{align*}
    X &= \left[
        x,\,
        y,\,
        z,\,
        \phi ,\,
        \theta ,\,
        \psi ,\,
        \dot{x} ,\,
        \dot{y} ,\,
        \dot{z} ,\,
        \dot{\phi} ,\,
        \dot{\theta} ,\,
        \dot{\psi} ,\,
        \ddot{x} ,\,
        \ddot{y} ,\,
        \ddot{z}
        \right]^\top
        \\
    X^+ &= f(X) = \left[
        x^+,\,
        y^+,\,
        \hdots,\,
        \ddot{z}^+
        \right]^\top
        \\
    x^+ &= x + \left(\dot{x}\cos{\psi}\cos{\theta}+ \dot{y}\left(\cos{\psi}\sin{\theta}\sin{\phi} - \sin{\psi}\cos{\phi}\right)+ \dot{z}\left(\cos{\psi}\sin{\theta}\cos{\phi} + \sin{\psi}\sin{\phi}\right)\right)\Delta_t \\ 
    &\qquad+ \frac{1}{2}\left(\ddot{x}\cos{\psi}\cos{\theta} + \ddot{y}\left(\cos{\psi}\sin{\theta}\sin{\phi} - \sin{\psi}\cos{\phi}\right) + \ddot{z}\left(\cos{\psi}\sin{\theta}\cos{\phi} + \sin{\psi}\sin{\phi}\right)\right)\Delta_t^2 \\
    y^+ &= y + \left(\dot{x}\sin{\psi}\cos{\theta} + \dot{y}\left(\sin{\psi}\sin{\theta}\sin{\phi} + \cos{\psi}\cos{\phi}\right) + \dot{z}\left(\sin{\psi}\sin{\theta}\cos{\phi} - \cos{\psi}\sin{\phi}\right)\right)\Delta_t\\
    &\qquad +\frac{1}{2}\left(\ddot{x}\sin{\psi}\cos{\theta} + \frac{1}{2}\ddot{y}\left(\sin{\psi}\sin{\theta}\sin{\phi} + \cos{\psi}\cos{\phi}\right) + \frac{1}{2}\ddot{z}\left(\sin{\psi}\sin{\theta}\cos{\phi} - \cos{\psi}\sin{\phi}\right)\right)\Delta_t^2 \\
    z^+ &= z + \left(-\dot{x}\sin{\theta} + \dot{y}\cos{\theta}\sin{\phi} + \dot{z}\cos{\theta}\cos{\phi}\right)\Delta_t + \frac{1}{2}\left(-\ddot{x}\sin{\theta} + \ddot{y}\cos{\theta}\sin{\phi} + \ddot{z}\cos{\theta}\cos{\phi}\right)\Delta_t^2 \\
    \phi^+ &= \phi + \left(\dot{\phi} + \dot{\theta}\sin{\phi}\tan{\theta} + \dot{\psi}\cos{\phi}\tan{\theta}\right)\Delta_t \\
    \theta^+ &= \theta + \left\left(\dot{\theta}\cos{\phi} - \dot{\psi}\sin{\phi}\right\right)\Delta_t \\
    \psi^+ &= \psi + \left(\dot{\theta}\frac{\cos{\phi}}{\cos{\theta}} + \dot{\psi}\frac{\sin{\phi}}{\cos{\theta}}\right)\Delta_t \\
    \dot{x}^+ &= \dot{x} + \ddot{x}\Delta_t \\
    \dot{y}^+ &= \dot{y} + \ddot{y}\Delta_t \\
    \dot{z}^+ &= \dot{z} + \ddot{z}\Delta_t \\
\end{align*}


==> chapters/stateestimation_synpf_rejected.tex <==
\section{State Estimation}

% Accurate and robust state estimation becomes crucial when autonomous mobile robots need to operate near their physical limits. This becomes apparent in our application, where maintaining control under rapid motion, operation near and  beyond the limits of traction, and physical proximity to track boundaries are decisive in achieving success. Two examples where this need is particularly prevalent are in the \textit{Control} and \textit{Perception} sections of the Race Stack depicted in \Cref{fig:sys_architecture}. In the Control section, an accurate state estimate is needed to determine appropriate control inputs. In the Perception section, the state estimate is crucial in classifying and predicting obstacle detections.

Accurate and robust state estimation is crucial for autonomous mobile robots. This becomes especially important when operating at the limits of traction. When observing the \emph{See-Think-Act} cycle depicted in \Cref{fig:sys_architecture}, it is clear that \emph{State Estimation} is the precursor to critical downstream tasks such as \emph{Perception}, \emph{Planning}, and \emph{Control}. These modules are intrinsically dependent on the quality of the state estimation data. Consequently, the accuracy and integrity of the state estimate are vital for the overall performance and safety of the racecar.

% PLAN \\
% x importance of fast and accurate state estimation in our setting, requirements \\
% x available signals (control odom, imu, scan) \\
% x role of localization, generating a prior - with TY \\
% Architecture Subsection: \\
% x description of EKF for prior \\
% x final combination of localization and EKF velocity estimates \\
% - potentially experimental validation or otherwise, limitations \\


\subsection{Architecture}
% Not entirely sure what to include. Here are a few ideas:
% covariance estimation? Fixed covariances for IMU?
% Frame definition?
% Illustrate point-mass model?
% define base-link; other frames?
% I saw the introduction has stuff about IO and UKF?

The task of state estimation is divided into localization and velocity estimation. The pipeline is depicted in \Cref{fig:se_loc_pipeline}. The sensor inputs used are linear accelerations and angular velocities from the \gls{imu}, a 2D laser scan from the \gls{lidar}, and \gls{erpm} odometry from the \gls{vesc} motor controller. The \gls{erpm} odometry is computed through the measured voltage within the \gls{vesc} motor controller, it is combined with the commanded steering angle to estimate the wheel odomtery using the implementation of the \emph{F1TENTH} platform presented in \cite{okelly2020f1tenth}, which can be significantly affected by tire-slip.

Within the \emph{State Estimation} module, an \gls{ekf} filtered odometry signal is fed to the localization algorithm, which is either \emph{Cartographer} \gls{slam} or a \gls{mcl}-based \gls{pf} algorithm specifically developed for racing, \emph{SynPF}. The localization algorithms are mutually exclusive. Lastly, the final car state is aggregated from the filtered odometry signal and the localization pose. The localization is done with respect to a pre-mapped racetrack, as further described in \Cref{chap:mapping}.

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/state_estimation.pdf}
    \caption{An overview of the proposed state estimation system architecture. The state estimation module incorporates velocity estimation and localization with respect to the pre-mapped racetrack and aggregates this information in a final car state odometry output both in Cartesian and in \emph{Frenet} coordinates.}
    \label{fig:se_loc_pipeline}
\end{figure}

%The accuracy of the odometry estimate, in particular the velocity components, has been found to significantly impact the performance of the localization through \emph{Cartographer} \gls{slam}, \todo{due to ...} \cite{synpf}.

% In order to supply sufficiently accurate velocity estimates, a filter-based approach is used.

Not only are sufficiently accurate velocity estimates required for the control algorithm, but localization performance is sensitive to the accuracy of the velocity components of the odometry prior. This odometry prior is especially critical when environmental conditions are exceptionally adverse towards accurate state estimation, as described in \Cref{chap:localization}. Therefore, a filter-based approach is used to improve the estimation accuracy of the velocity states by combining multiple sensor modalities, as described in \Cref{chap:ekf}.

In contrast, direct velocity estimation by performing finite differencing on localization data is impractical. Firstly, localization estimates may exhibit spatial discontinuity or jitter, which would lead to noisy velocity estimates. More importantly, localization estimates have latency, which results in delayed velocity estimates, whereas in the proposed setup the estimated values lag the true values by around \qty{0.5}{\second}. This is not desirable in a racing scenario, as such inaccurate velocity estimates would inevitably lead to downstream components performing poorly.

% Therefore, the \emph{Odom Filter} employs a point-mass \gls{ekf} to supply the localization algorithm with a refined and consistent prior. This approach not only enhances the smoothness and accuracy of the localization but also delivers a reliable velocity estimate.

% The Localization component, detailed in \Cref{chap:localization}, estimates the vehicle's pose in the global frame given the current sensor inputs. The Velocity Estimation component estimates the linear and angular velocities of the vehicle and consists of an \gls{ekf}, detailed in \Cref{chap:ekf}.

% In the ultimate step of the state estimation pipeline, the filtered velocity state estimate and the pose estimate are concatenated to form a complete odometry estimate. The resultant car state estimate is outputted at a rate of \qty{80}{\hertz}.

\subsection{Odometry Filter - Extended Kalman Filter} \label{chap:ekf}

% for example when track boundaries offer low reflectivity, degrading the \gls{lidar} signal, or when the track surface provides reduced traction (not sure if I should mention this, as this paper doesn't address this issue I think).

Velocity state estimates are generated using an approach based on the \gls{ekf} \cite{Kalman1960}. It fuses the wheel odometry and the data provided by the \gls{imu} sensor. This aids the robot in situations where tire slip occurs, as the accelerometer data from the \gls{imu} can be leveraged to compensate for this within the \gls{ekf}. The \gls{ekf} is integrated through the \texttt{robot\_localization} package \cite{robotlocalization}. The estimates are generated at a rate of \qty{50}{\hertz}, corresponding to the \gls{imu} update frequency.

The \gls{ekf} model consists of an omnidirectional, two-dimensional point-mass motion model. The states that can be estimated using this approach are therefore the longitudinal velocity, lateral velocity, and the yaw rate. However, if no lateral acceleration data is supplied to the motion model, the vehicle's lateral velocity is assumed to be \qty{0}{\meter\per\second}, which is equivalent to assuming that the vehicle experiences no lateral slip. While more vehicle-specific motion models have been investigated, this approach was observed to be more robust to significantly varying track conditions than the implemented vehicle-models, and performed sufficiently well under \emph{realistic} driving conditions.

As outlined in the documentation of the \gls{ekf} package \cite{robotlocalization}, the a posteriori update step of the \gls{ekf} can be configured by selecting the specific measurement sources from each sensor or input to be considered. Furthermore, the filter can be easily expanded with data from additional sensors using this configuration, enabling and encouraging future investigation in this area.

The ideal fusion configuration is determined experimentally using ground-truth motion capture data and qualitative observations, as described in \Cref{chap:SE_results}. In the selected configuration, the \gls{ekf} fuses the \gls{imu} measurements of angular velocity, heading, and the full twist stemming from the wheel odometry. Note that linear accelerations observed by the \gls{imu} sensor are not considered, as they were observed to experience significant noise due to shaking and may be sensitive to the exact positioning and orientation of the \gls{imu} sensor on the car. Nevertheless, the configuration of \gls{ekf} inputs can be changed quickly and easily to maximize the estimation accuracy given the external conditions.

The covariances associated with the individual measurements are determined at their respective sources, and are used in forming the measurement update of the \gls{ekf}. In this implementation, the covariances of the \gls{imu} data and the control odometry are predetermined and set to be static.

\subsection{Localization} \label{chap:localization}
Accurate localization is important, due to the trickle-down effects on the rest of the \emph{ForzaETH Race Stack}. Therefore, the proposed \emph{Race Stack} supports two mutually exclusive options for localization to suit varying conditions:

\begin{enumerate}[I]
    \item \textbf{Cartographer:} A pose-graph optimization \gls{slam} method \cite{loc_cartographer}. This localization method yields the most accurate and smoothest pose estimate, given high-quality odometry input data. This localization technique works very well, as long as the racecar experiences relatively low levels of tire slip, such that the wheel odometry signal is sufficiently accurate. It is a \gls{cpu} bound algorithm which is responsible for 67.5\,\% of \gls{cpu} utilization of the \emph{Race Stack}.

    \item \textbf{SynPF:} A high-performance \gls{mcl}-based \gls{pf} localization technique optimized for racing, specifically developed for the \emph{ForzaETH Race Stack}. As opposed to \emph{Cartographer}, this method yields slightly less accurate pose estimates with higher jitter. This lack of accuracy may be due to the approximations used. However, this method is highly robust against low-quality odometry input. In a racing environment with high levels of wheel slip, \emph{SynPF} is a very performant localization alternative. Furthermore, \emph{SynPF} is computationally lighter, responsible for 55.3\,\% of \gls{cpu} utilization of the \emph{Race Stack}. This is because it can be offloaded to memory by utilizing a \gls{lut}, or it can be computed in parallel on an available \gls{gpu}.
\end{enumerate}

An additional critical aspect to consider next to the localization accuracy is the robustness of the State Estimation pipeline to the quality of odometry input. In racing scenarios, wheel-slip is a frequent occurrence, especially on slippery surfaces. This slip can significantly degrade the quality of wheel odometry, which serves as a prior for the localization subsystem. Given the contrasting strengths of each localization method (all-out performance versus robustness), operators can decide which one to use given the conditions at each race event. The different performance characteristics between \emph{Cartographer} and \emph{SynPF} given high- and low-quality odometry input are illustrated in \Cref{fig:localization-method-pros-cons}. Specifically, \Cref{fig:badodom_icra22} demonstrates the catastrophic failure case of \emph{Cartographer} \gls{slam}, which could not handle the compromised odometry signal, leading to a collision against the track's right barrier, as evidenced by the \gls{lidar} scans. In contrast, \emph{SynPF} was able to accurately localize using the same dataset.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/SE/state_estimation_good_bad_odom.pdf}
    \caption{A comparison of the supported localization methods, \emph{Cartographer} and \emph{SynPF}. \textbf{Left:} Nominal conditions showing high-quality odometry. \textit{Cartographer} publishes pose estimates at a higher frequency than \emph{SynPF}, shown by the more densely-spaced data points along its reported trajectory. \textbf{Right:} Low-grip conditions with wheel spin. \textit{Cartographer} is unable to provide an accurate pose estimate, estimating that the racecar is in the middle of the track, while in reality, it has crashed into the boundaries. However, \textit{SynPF} operates nominally, correctly estimating the racecar's actual position. This comparison was made possible by retrospectively applying the \emph{SynPF} algorithm to telemetry data recorded during the car's operation with \emph{Cartographer}.}
    \label{fig:localization-method-pros-cons}
\end{figure}

\begin{comment}
% This is from the original plot
\includegraphics[trim=0 0 0 0cm, clip, width=0.48\textwidth]{figures/SE/ScanAlignFigures/slam_bad.png}
\hfill % This adds a little space between the images
\includegraphics[trim=0 0 0 0cm, clip, width=0.48\textwidth]{figures/SE/ScanAlignFigures/synpf_bad.png}
\end{comment}

\begin{figure}[ht]
    \centering
    \includegraphics[trim=0 0 0 0cm, clip, width=\textwidth]{figures/SE/ScanAlignFigures/scan_align_fig.pdf}
    \caption{Low-quality odometry conditions corresponding to the right side of \Cref{fig:localization-method-pros-cons} showcasing both \emph{Cartographer} and \emph{SynPF} under worst-case conditions in four sequential time steps, indicated with $t_i$. At $t_2$, \emph{Cartographer} is unable to align the \gls{lidar} scans with the track boundaries, while \emph{SynPF} maintains a visibly steady track alignment.}
    \label{fig:badodom_icra22}
\end{figure}

\FloatBarrier

\subsection{\emph{SynPF} Implementation Details} \label{chap:synpf-impl-details}

\emph{SynPF} synthesizes ideas from several previous \gls{pf} methodologies, optimizing them for high-performance, low-latency operation. These improvements focus on the \emph{motion model} and \emph{sensor model} of the \gls{pf} algorithm.

For the \emph{motion model}, improving its formulation improves \emph{particle efficiency}, whereby each particle better represents the physically probable motions of the racecar. This means fewer particles are needed, reducing computation time. Here, \emph{SynPF} employs an improvement to the \emph{diff-drive} motion model \cite{loc_probabilisticrobotics} by TUM \cite{tum-pf}. This formulation caps how much angular uncertainty may be scaled by the longitudinal velocity of the racecar. This is because at high velocities, for instance on straight sections of a racetrack, the car’s angular uncertainty is low, as the steering input cannot be large.

For the \emph{sensor model}, a majority of computation effort in \gls{mcl} methods is in evaluating the expected sensor range at a given pose. This is accelerated by using the \verb|rangelibc| \cite{MIT_PF} library. It allows the use of an available \gls{gpu} to parallelize a ray-casting operation over all selected scan-lines, vastly accelerating the calculation of the expected ranges. In addition, it also offers a \gls{lut} option to pre-calculate all expected ranges for a discretized set of poses in the map, resulting in constant-time query speed at the expense of memory usage. Utilizing one of the two methods greatly increases the rate at which the sensor model can be evaluated.

\subsection{Localization Parameters}
Both the \emph{Cartographer} and \emph{SynPF} algorithms were tuned to minimize the lap time in a \emph{Time-Trials} scenario over multiple maps. The parameters are shown as \verb|[min, max, tuned]|:

\begin{enumerate}[I]
    \item \textbf{Cartographer:}
    The parameters are identical to those in \Cref{item:mapping_slam_params}. However, \emph{Cartographer} is now run in \emph{localization-only} mode, which runs with lower latency and compute usage, as it uses the previously generated map of the racetrack.

    \item \textbf{SynPF}
    These parameters affect the variance of noise applied to the \emph{SynPF} motion model and correspond to those in \cite{tum-pf}.

    \begin{itemize}
        \item \texttt{$\alpha_{1}$} \verb|[0.0, 1.0, 0.5]| - how much rotation affects rotation variance.
        \item \texttt{$\alpha_{2}$} \verb|[0.0, 0.05, 0.01]| - how much translation affects rotation variance.
        \item \texttt{$\alpha_{3}$} \verb|[0.0, 1.0, 0.1]| - how much translation affects translation variance.
        \item \texttt{$\alpha_{4}$} \verb|[0.0, 5.0, 1.0]| - how much rotation affects translation variance.
        \item \texttt{lam\_thresh} \verb|[0.01, 0.2, 0.1]| - minimum translation for the TUM model to become effective.
    \end{itemize}
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{State Estimation Results} \label{chap:SE_results}

This section evaluates the accuracy of various state estimation frameworks against ground truth data, primarily using a motion-capture system for validation. The test vehicle was equipped with reflective markers and navigated autonomously on a specially designed track. Positional data was recorded from the motion-capture system alongside the vehicle's sensor and control data. This comprehensive dataset enables offline analysis of different state estimation frameworks, including the two localization algorithms previously discussed. \Cref{fig:VICON} illustrates the experimental setup.

\begin{figure}[ht]
    \centering
    %\includegraphics[width=0.46\textwidth]{figures/SE/IMG_3826.jpg}
    %\includegraphics[width=0.46\textwidth]{figures/SE/VICON_markers_placeholder.jpg}
    \includegraphics[width=\textwidth]{figures/SE/VICON_PVC.pdf}
    \caption{Experimental setup with a motion capture system. Reflective markers are fitted to the car. This allows for millimeter accuracy ground truth tracking at frequencies up to \SI{100}{\hertz}.}
    \label{fig:VICON}
\end{figure}

However, to assess the localization accuracy with respect to the quality of the wheel odometry signal, the motion capture system's limited coverage on larger tracks, coupled with the challenges of capturing wheel-slip effects at the edge of traction, necessitated the use of alternative quantitative measures in certain experiments. These include lap time analysis and lateral deviation from the ideal racing line, which serve as proxy measurements for localization accuracy. While indirect, these metrics are crucial indicators of localization accuracy, which in turn significantly impacts the vehicle's performance and safety. Ultimately, in a racing context, these factors converge on the final lap time, a critical measure of success. \Cref{fig:quant_tracks} illustrates the test track used for these evaluations. The track features high-quality wheel odometry under normal tire conditions (\SI{26}{\newton} lateral force), and low-quality wheel odometry when the tires are modified with tape (\SI{19}{\newton} lateral force), as confirmed by a spring force meter measuring the maximum lateral force applicable to the stationary racecar.

Additionally, we assess the effectiveness of the localization algorithms by examining scan alignment. This involves calculating the ratio of points falling within a predefined distance from the track boundaries. A lower score in this metric would indicate a notable decline in localization accuracy, underscoring the importance of precise state estimation in high-speed racing scenarios.

\begin{figure}[ht]
    \centering
    \includegraphics[trim={0cm 0 0cm 25cm}, clip, width=0.46\textwidth]{figures/currywurst.jpg}
    \includegraphics[trim={0cm 0 0 0}, clip, width=0.46\textwidth]{figures/slippery_tires.png}
    \caption{Test track used for quantitative localization accuracy evaluations. Left: Grippy track providing high-quality odometry readings. Right: Car with modified tires to increase slipperiness which yields less accurate wheel odometry data.}
    \label{fig:quant_tracks}
\end{figure}

\subsubsection{Localization Accuracy} \label{chap:localization_results}
\Cref{fig:vicon-pf-slam-results} quantifiably shows that \emph{Cartographer} is capable of delivering accurate pose estimates, especially with the high-quality wheel odometry inputs in the given scenario, with an average RMSE of \SI{0.0535}{\meter}. However, the limited area coverage of the motion capture system necessitated a small racetrack setup. \emph{SynPF} struggles to give accurate localization in this scenario, with a higher RMSE of \SI{0.1998}{\meter}.

However, it should be stressed that the racetrack setup with the motion capture system is very small compared to a competition scenario. Furthermore, to assess the localization performance with respect to the quality of the wheel odometry signal, larger racetracks are needed. This is particularly necessary in order to capture wheel-slip effects at the edge of traction. Therefore, alternative quantitative measures are used, detailed in \Cref{sec:localization_robustness}.

Firstly, the lap times and lateral deviation from the racing line planned in \Cref{subsec:gb_optimizer} are used as proxy measurements for the overall performance of the localization algorithm with respect to the quality of the wheel odometry signal. While indirect, these metrics converge on the final lap time, a critical measure of success in a racing scenario, especially in the \emph{Time-Trials} phase of the competition.

Secondly, the effectiveness of the localization algorithms is assessed by examining scan alignment. This involves calculating the ratio of points falling within a predefined distance from the track boundaries. A lower score in this metric would indicate a notable decline in localization accuracy, underscoring the importance of precise state estimation in high-speed racing scenarios.

\subsubsection{Localization Robustness} \label{sec:localization_robustness}
\Cref{tab:combined_quant_results} holds the resulting accuracy proxy measurements for \emph{Cartographer} and \emph{SynPF} under the influence of varying odometry quality. \emph{SynPF} shows an approximately \SI{0.15}{\second} faster lap time in the low-quality odometry scenario and a significantly lower lateral deviation of \SI{7.68}{\centi\metre} as opposed to \emph{Cartographer}'s \SI{11.43}{\centi\metre} error.
On the other hand, when performing the same experiment on the test track under favorable grippy (high-quality) odometry conditions, \Cref{tab:combined_quant_results} showcases that the high-quality odometry signal allows \emph{Cartographer} to perform a roughly \SI{0.02}{\second} faster average lap time than \emph{SynPF} with a lower lateral error of \SI{6.86}{\centi\metre}, as opposed to \emph{SynPF}'s \SI{8.22}{\centi\metre} error.
Interestingly to note, is that for \emph{Cartographer} the lateral error increases by 67\%, from \SI{6.86}{\centi\metre} to \SI{11.43}{\centi\metre} when going from high to low-quality odometry, while for \emph{SynPF} the change is merely 6.9\% from \SI{8.22}{\centi\metre} to \SI{7.68}{\centi\metre}.
Further, the scan alignment score demonstrates that the proposed \emph{SynPF} algorithm significantly outperforms \emph{Cartographer} when set in a low-quality odometry setting (79.92\% vs 61.71\%), by yielding a factor 1.29 better scan alignment ratio. Therefore, it can be seen that with a grippy and high-quality odometry signal the \gls{slam} method yields a marginally lower lap time and lower lateral error, while, under slippery conditions, the \gls{mcl}-based \emph{SynPF} algorithm yields significantly better racing performance. To summarise, \emph{Cartographer}'s performance deteriorates when conditioned in low-quality odometry by -11.0\% in average scan alignment and +66.6\% in lateral error, while \emph{SynPF} exhibits robustness to low-quality odometry and showcases a significantly lower deterioration with a mere -0.08\% scan alignment and -6.9\% lateral error while still maintaining very competitive lap times.

% In both cases, \emph{SynPF} shows a higher average lateral error to the pre-computed racing line. This results from the pose estimate of \emph{SynPF} only being an approximation, due to the sampling nature of \gls{mcl} algorithms. These less exact pose estimates from \emph{SynPF} may result in the control of the car not performing as well as when \emph{Cartographer} is used, which results in a larger lateral error.

\begin{table}[ht]
\centering
\setlength{\tabcolsep}{1.5pt} % Reduces the padding between columns
\renewcommand{\arraystretch}{1.5} % Increases the row height
\begin{tabular}{c|c|c|c|c|c|c}
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Odom}} & \multicolumn{2}{c|}{\textbf{Lap Time [s]}} & \multicolumn{2}{c|}{\textbf{Error [cm]}} & \multirow{2}{*}{\parbox[c]{1.475cm}{\centering \textbf{Scan} \\ \textbf{Align [\%] $\uparrow$}}} \\
& & $\mu$ $\downarrow$ & $\sigma$ $\downarrow$ & $\mu$ $\downarrow$ & $\sigma$ $\downarrow$ & \\
\hline
\hline
\multirow{2}{*}{\emph{Cartographer}} & HQ & \textbf{9.167} & \textbf{0.097} & \textbf{6.864} & \textbf{0.264} & 69.357\\
& LQ & 9.428 & 0.126 & 11.432 & \textbf{1.134} & 61.710\\
\hline
\multirow{2}{*}{\emph{SynPF}} & HQ & 9.184 & 0.153 & 8.223 & 0.406 &\textbf{80.603} \\
& LQ & \textbf{9.280} & \textbf{0.093} & \textbf{7.686} & 1.179 & \textbf{79.924} \\
\end{tabular}
\caption{Lap time and computation results on the test track of \Cref{fig:quant_tracks}, featuring slippery (low-quality: LQ) and grippy (high-quality: HQ) odometry input. The average lateral error is with respect to the ideal racing line. The scan alignment score is computed by the average percentage of overlapping scans and the track boundary. The compute metric refers to \texttt{htop} percentage of \gls{cpu} core utilization.}
\label{tab:combined_quant_results}
\end{table}

\begin{comment}
\subsubsection{Velocity Estimation Accuracy}
The velocity state estimate trajectories produced by the frameworks in question are depicted in \Cref{fig:results_SE_1}. The algorithm was executed for approximately one minute in order to calculate performance metrics, while the trajectories were plotted for a reduced time corresponding to two laps of the test track.

To further illustrate the differences between \emph{Cartographer} and \emph{SynPF}, as well as their effectiveness, we evaluate these algorithms by running them offline on data recorded during official F1TENTH competitions in conditions featuring grippy and slippery floors, thus creating both high- and low-quality odometry data. This means algorithms can be compared on the exact same data, as it can be very difficult to replicate slipping behaviour that results in a visible localization failure due to the time-series data dependencies of both algorithms. The tracks used are shown in \Cref{fig:icra_tracks}.

\begin{figure}[ht]
    \centering
    \includegraphics[trim=0 0 0 15cm, clip, width=0.43\textwidth]{figures/ICRA23Track1.jpg}
    \label{fig:icra23}
    \includegraphics[trim=0 0 0 0, clip, width=0.43\textwidth]{figures/ICRA22Track1.png}
    \label{fig:icra22}
    % \vspace*{-4mm}
    \caption{Conditions for localization. Left: Grippy floor yields high-quality odometry at the ICRA23 race. Right: Slippery polished concrete yields low-quality odometry at the ICRA22 race.}
    \label{fig:icra_tracks}
\end{figure}

To compare localization algorithms, \textit{scan alignment} was used. This is calculated by superimposing the measurements from the \gls{lidar} on the reported pose from the localization algorithm. These points are then checked for alignment with the known map boundaries. A higher agreement between these superimposed measurements and the map boundaries indicates higher localization accuracy.

\Cref{fig:goododom_icra23} illustrates the scan alignment of \emph{SynPF} and \emph{Cartographer} given high-quality odometry data. Unsurprisingly, both methods yield a high score. While at $t_1$, \emph{Cartographer} may have a lower scan alignment score of \qty{83.89}{\%} compared to \qty{100.0}{\%} by \emph{SynPF}, note that its other desirable properties of smooth, high-frequency pose estimates give it the overall edge in this scenario.

\begin{figure}[ht]
    \centering
        \includegraphics[trim=0 3.7cm 0 0, clip, width=0.45\textwidth]{figures/SE/ScanAlignFigures/slam_good.png}
        \label{fig:slam_goododom_icra23}

        \includegraphics[trim=0 3.7cm 0 0cm, clip, width=0.45\textwidth]{figures/SE/ScanAlignFigures/synpf_good.png}
        \label{fig:pf2_goododom_icra23}
    \caption{High-quality odometry conditions on the ICRA23 racetrack. The figure showcases both \gls{slam} and \emph{SynPF} under best-case conditions in two sequential time steps, indicated with $t_1,\,t_2$. Both algorithms perform reasonably well, as the \gls{lidar} scans visibly align well with the track boundaries.}
    \label{fig:goododom_icra23}
\end{figure}

\Cref{fig:badodom_icra22} illustrates the scan alignment of \emph{SynPF} and \emph{Cartographer} low-quality odometry data. The presence of wheel slip means that the odometry distance reported is larger than the actual distance covered by the racecar. This scenario is made even more difficult by the lack of distinctive features from the \gls{lidar} sensor, as the racecar is travelling along a straight section of the racetrack.

With lack of information from both \gls{lidar} and odometry, \emph{Cartographer} is unable to cope with this biased data, showing scan misalignment at $t_2$ in \Cref{fig:badodom_icra22}. Yet, due to its sampling-based nature, \emph{SynPF} can still yield an accurate pose estimate.

\begin{figure}[ht]
    \centering
        \includegraphics[trim=0 3.8cm 0 0cm, clip, width=0.45\textwidth]{figures/SE/ScanAlignFigures/slam_bad.png}
        \label{fig:slam_badodom_icra22}

        \includegraphics[trim=0 3.8cm 0 0cm, clip, width=0.45\textwidth]{figures/SE/ScanAlignFigures/synpf_bad.png}
        \label{fig:pf2_badodom_icra22}
    \caption{Low-quality odometry conditions on the ICRA22 racetrack showcasing both \emph{Cartographer} and \emph{SynPF} under worst-case conditions in two sequential time steps, indicated with $t_1,\,t_2$. This highlights the robustness properties of \emph{SynPF} to deteriorating odometry quality. At $t_2$, \emph{Cartographer} is unable to align the \gls{lidar} scans with the track boundaries, while \emph{SynPF} maintains a visibly steady track alignment.}
    \label{fig:badodom_icra22}
\end{figure}

\begin{figure}[ht]
    \centering
    \begin{minipage}{0.475\textwidth}
        \centering
        \includegraphics[width=7.5cm]{figures/SE/2023-08-12-17-45-23_velocity_long.pdf}
        \includegraphics[width=7.5cm]{figures/SE/2023-08-12-17-45-23_x_position.pdf}
    \end{minipage}\hfill
    \begin{minipage}{0.475\textwidth}
        \centering
        \includegraphics[width=7.5cm]{figures/SE/2023-08-12-17-45-23_yaw_rate.pdf}
        \includegraphics[width=7.5cm]{figures/SE/2023-08-12-17-45-23_y_position.pdf}
    \end{minipage}\hfill
    \caption{State estimation curves for cartesian coordinates, longitudinal velocity, and yaw rate corresponding to one lap around the test track. The two different localization techniques available are compared against ground-truth data.}
    \label{fig:results_SE_1}
\end{figure}

%With the integrated method, it is possible to estimate the longitudinal and angular velocity with estimation accuracies of approximately \qty{0.194}{\meter\per\second} and \qty{0.114}{\radian\per\second} \gls{rmse}, respectively. 
The \gls{rmse} have been determined for each of the odometry states, using each of the available localization frameworks, as summarized in \Cref{tab:SE_rmse}.

\begin{table}[ht]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
         & \textbf{${v_{lon}}$} & \textbf{$v_{lat}$} & \textbf{$v_\psi$} & \textbf{$s$} & \textbf{$d$} & \textbf{$\psi$} \\
        \emph{Configuration} & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ \\
         & [\unit{\metre\per\second}] & [\unit{\metre\per\second}] & [\unit{\radian\per\second}] & [\unit{\meter}] & [\unit{\meter}] & [\unit{\radian}] \\
        \hline
        \hline
        \emph{Odom Filter} + \emph{Cartographer} & 0.2309 & \textbf{0.0772} & 0.0943 & 0.1039 & \textbf{0.0606} & \textbf{0.0316} \\
        \emph{Odom Filter} + \emph{SynPF} & \textbf{0.2275} & \textbf{0.0772} & \textbf{0.0808} & \textbf{0.0887} & 0.1037 & 0.0552 \\
    \end{tabular}
    \caption{State estimation accuracies of various odometry states while driving several laps around the test track as evaluated against motion capture data on the track setup outlined in \Cref{chap:SE_results}.}
    \label{tab:SE_rmse}
\end{table}

\end{comment}

\subsubsection{Velocity Estimation Accuracy}
The state estimation accuracy of various frameworks was evaluated against ground truth data acquired using a motion-capture system. The car was fitted with reflective markers and driven autonomously on a test track. Positional data from the motion-capture system was recorded, in addition to the sensor and control data provided by the vehicle. This allows for the various state estimation frameworks, including the two aforementioned localization algorithms, to be run offline. The experimental setup is depicted in \Cref{fig:VICON}.

\begin{figure}[ht]
    \centering
    \begin{minipage}{0.43\textwidth}
        \vspace{-1.1em}
        \centering
        \includegraphics[width=\textwidth]{figures/SE/trajectories.pdf}
        \caption{On the small racetrack set up with the motion capture system, \emph{Cartographer} is well able to closely match the ground-truth trajectory, while \emph{SynPF} performs slightly worse.}
        \label{fig:vicon-pf-slam-results}
    \end{minipage}\hfill
    \begin{minipage}{0.54\textwidth}
        \centering
        \includegraphics[width=0.49\textwidth]{figures/SE/2023-08-12-17-45-23_velocity_long.pdf}
        \includegraphics[width=0.49\textwidth]{figures/SE/2023-08-12-17-45-23_x_position.pdf}
        \includegraphics[width=0.49\textwidth]{figures/SE/2023-08-12-17-45-23_yaw_rate.pdf}
        \includegraphics[width=0.49\textwidth]{figures/SE/2023-08-12-17-45-23_y_position.pdf}
        \caption{State estimation curves for cartesian coordinates, longitudinal velocity, and yaw rate corresponding to one lap around the test track. The two different localization techniques available are compared against ground-truth data.}
        \label{fig:results_SE_1}
    \end{minipage}
\end{figure}

The velocity state estimate trajectories produced by the frameworks in question are depicted in \Cref{fig:results_SE_1}. The algorithm was executed for approximately one minute in order to calculate performance metrics, while the trajectories were plotted for a reduced time corresponding to two laps of the test track. The \gls{rmse} have been determined for each of the odometry states, using each of the available localization frameworks, as summarized in \Cref{tab:SE_rmse}.

\begin{table}[ht]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
         & \textbf{${v_{lon}}$} & \textbf{$v_{lat}$} & \textbf{$v_\psi$} & \textbf{$s$} & \textbf{$d$} & \textbf{$\psi$} \\
        \emph{Configuration} & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ & \gls{rmse} $\downarrow$ \\
         & [\unit{\metre\per\second}] & [\unit{\metre\per\second}] & [\unit{\radian\per\second}] & [\unit{\meter}] & [\unit{\meter}] & [\unit{\radian}] \\
        \hline
        \hline
        \emph{Odom Filter} + \emph{Cartographer} & 0.2309 & \textbf{0.0772} & 0.0943 & 0.1039 & \textbf{0.0606} & \textbf{0.0316} \\
        \emph{Odom Filter} + \emph{SynPF} & \textbf{0.2275} & \textbf{0.0772} & \textbf{0.0808} & \textbf{0.0887} & 0.1037 & 0.0552 \\
    \end{tabular}
    \caption{State estimation accuracies of various odometry states while driving several laps around the test track as evaluated against motion capture data on the track setup outlined in \Cref{chap:SE_results}.}
    \label{tab:SE_rmse}
\end{table}

